Ornstein Isomorphism and Algorithmic Randomness

In 1970, Donald Ornstein proved a landmark result in dynamical systems, viz., two Bernoulli systems with the same entropy are isomorphic except for a measure 0 set. Keane and Smorodinsky gave a finitary proof of this result. They also indicated how one can generalize the result to mixing Markov Shifts. We adapt their construction to show that if two computable mixing Markov systems have the same entropy, then there is a layerwise computable isomorphism defined on all Martin-Lof random points in the system. Since the set of Martin-Lof random points forms a measure 1 set, it implies the classical result for such systems. This result uses several recent developments in computable analysis and algorithmic randomness. Following the work by Braverman, Nandakumar, and Hoyrup and Rojas introduced discontinuous functions into the study of algorithmic randomness. We utilize Hoyrup and Rojas' elegant notion of layerwise computable functions to produce the test of randomness in our result. Further, we use the recent result of the effective Shannon-McMillan-Breiman theorem, independently established by Hochman and Hoyrup to prove the properties of our construction. We show that the result cannot be improved to include all points in the systems - only trivial computable isomorphisms exist between systems with the same entropy.

==> 3.intermediate_construction.tex <==
\section{Layerwise lower semicomputable isomorphism between processes with equal
  entropy}

In this section, we provide the proof of Theorem 1. We will construct
an isomorphism and establish that it is layerwise lower
semicomputable. We will elaborate on the overview presented in section
3. The proof is structured in sections, as in the presentation of the
Keane-Smorodinksy proof.

Now, we proceed with the stages of the algorithm.

\subsection{An Effective  Marker Lemma}
We want to construct an isomorphism between two mixing Markov systems
\A and \B with equal entropy. We will construct an intermediate mixing
Markov system \C with a finite alphabet $\Sigma_C$ and computable
probability. We designate two symbols $0$ and $1$. We aim to construct
an intermediate system \C so that all cylinders $x\in\{0\}^*$ in
system \A have the same probability as the cylinder $x$ in the system
\C and similarly all cylinders $y\in\{1\}^*$ in the system \B have the
same probability as the cylinder $y$ in system \C.

If we can construct such an intermediate system, then we show that the
problem reduces to mapping each cylinder in one system to a cylinder
of same length in the other. %% i.e., the
%% designated symbol acts as a framework for cylinder and cylinder
%% decompositions ( called skeletons ). 
Let $I_1$ be the layerwise lower semicomputable isomorphism between \A
and \C and $I_2$ be the layerwise lower semicomputable isomorphism
between \B and \C. The final isomorphism between \A and \B is $I_1
\circ I_2^{-1}$. Note that the composition of layerwise lower
semicomputable functions need not be layerwise lower semicomputable in
general, however our composition of isomorphisms $I_1 \circ I_2^{-1}$
preserves layerwise lower semicomputability.

Consequently, the final isomorphism also maps a cylinder to a cylinder
of same length. We construct the intermediate system \C in such a way
that given a finite cylinder of a Martin-L\"of random sequence in \A,
we can determine the central coordinate of the image in a computably
enumerable manner.


\subsubsection{Construction of the intermediate system}
 Observe that we can assume without loss of generality that both
 $\Sigma_A,\Sigma_B$ alphabets has at least 3 symbols and all symbols
 in $\Sigma_A$ and $\Sigma_B$ have probability less than
 $1/4$.\footnote{Otherwise consider systems with alphabets
   $\Sigma_A^n$ and $\Sigma_B^n$ and ergodic transformations $T_1^n$
   and $T_2^n$ for sufficiently large $n$. It is easy to see that the
   new systems are also Markov and both the systems have same entropy
   $nH$.  Further, a layerwise lower semicomputable isomorphism
   between new systems trivially yields such an isomorphism between
   the original systems.}

To determine the intermediate system, first we need to fix an alphabet
$\Sigma_C$.  Then we need to construct a Turing machine $M_C$ which,
on input $x\in\Sigma_C^*$ and $n\in\N$, returns the probability of
cylinder $x$ in \C within error of $\varepsilon_n$.  We require that
the probabilities thus computed satisfy the following.
\begin{enumerate}
  \item For $x \in \{0\}^*$, $P_A(x) = P_c(x)$, and for $y \in
    \{1\}^*$, $P_B(y) = P_C(y)$.
  \item $H(\C) = H(\A) = H(\B)$.
  \item \C is a mixing Markov process with memory $m$.
\end{enumerate}

First we determine the size of $\Sigma_C$. Sort the symbols $a \in 
\Sigma_A$ and $b \in \Sigma_B$ in descending
order with respect to $P_A(a,3)$ and $P_B(b,3)$ respectively.
Designate a symbol in $\Sigma_A$ with the largest probability as $0$
and a symbol in $\Sigma_B$ with the least probability as $1$. Note
that we are assured that $P_C(\Sigma_C \setminus \{0,1\}) > \frac{1}{4}$. Let
$c'$ be the smallest natural number so that $\frac{1}{4}\log(c'-2) \ge
(H+1)$. Let $c=\max(c',|\Sigma_A|,|\Sigma_B|)$. We define $\Sigma_C$
to be $\{0, 1, \dots, c\}$.

Now we outline the algorithm $M_C$ for computing the probability
$P_C$. Let the input string be $x \in \Sigma_C^*$. We can easily
satisfy condition 1: $M_C(x,n) = M_A(x,n)$ when $x \in \{0\}^*$
and returns $M_C(x,n) = M_B(x,n)$ when $x \in \{1\}^*$. For other
inputs, we construct the probabilities by induction on the error
bound. %We give a rough outline as to how $M_C(x,n)$ works.

If $|x| \le m+1$, then we do the following. Let, for every $z \in
\Sigma_C^{m+1}$, $P(z)$ be $M_C(z, n-1)$. While either $|H(P)-H(A)|$
or $|H(P)-H(B)|$ is greater than $\epsilon_n$, we adjust, for strings
$z \in \Sigma_C^{m+1}$ in steps of $P(z)\varepsilon_n$ so that
$\max\{|H(P)-H(A)|, |H(P)-H(B)|\}$ strictly decreases while maintaining
that new probability is consistent with $P(z,k)$ for $1\le k\le n-1$.
This is always possible -- the maximum entropy of a distribution on 
$\Sigma_C^{m+1}$ is 
$$(m+1) c\;>\; \max \{ 4(m+1)(H+1),\ (m+1)\log |A|,\ (m+1)\log
|B|\},$$ which is at least as large as the maximum possible entropies
of $\Sigma_A^{m+1}$ and $\Sigma_B^{m+1}$, and the minimum possible
entropy of a distribution on $\Sigma_C^{m+1}$ with $P_C(0)$ and
$P_C(1)$ fixed appropriately, is $(m+1) \left[ -2\times \frac{1}{4}
  \log_2 \frac{1}{4} - \frac{1}{2} \log \frac{1}{2} \right]$, which
matches the minimum possible entropy of $\Sigma_A^{m+1}$ and
$\Sigma^{m+1}_B$. Since entropy is a continuous function of the
probability vector, by making adjustments to the probabilities on
$\Sigma_C^{m+1}$, it is possible to attain a probability vector $P$ on
$\Sigma_C^{m+1}$ such that $|H(P) - H| < (m+1)\epsilon$.
Although this $P$ might real valued, we are approximating within
$\epsilon_n$ in $P_C(\cdot,n)$.



If the input string $x$ contains more than $m+1$ characters, we first
assign, for every $z \in \Sigma_C^{m+1}$, $P(z) = M_C(z, n|x|)$. Now,
for every symbol $a \in \Sigma_C$ and string $y \in \Sigma^m_C$, we
let 
$$P(a \mid y) = \frac{P(y a)}{ \sum_{c \in \Sigma_C} P(y c)}.$$
Now, compute 
$$P(x[1 \dots q]) = P(x[1 \dots m]) \prod_{i=m+1}^{q}
P\left(x[i]\,\mid\,x[i-m \dots i-1]\right).$$
It is clear that the constructed process is a mixing Markov process
with memory $m$.

%{\bf Changelog: What is $y^r$? $r=1$.}

From the construction, it is clear that the system \C thus constructed
has a same entropy as that of \A and \B. Also, it is clear from the
construction that \C is a stationary mixing Markov with memory $m$.
Note that we also compute $P_C(a|x,n)$  in the process of computing
$P_C(\cdot,n)$.

Note that $P(z,n)$ for $z\in\Sigma_C^k$ is not a valid probability 
distribution -- in particular ``probabilities'' may not add up to $1$.
But for the purpose of our construction it is immaterial.


%% TeX-Master=markov.tex
 

%%  LocalWords:  Layerwise semicomputable layerwise Smorodinksy nH
%%  LocalWords:  semicomputability


==> 4.skeleton_lemma.tex <==
\subsection{An Effective Skeleton Lemma}
We can now consider two systems \A and \C with $P_A(0) = P_C(0)$. We
will now consider those pairs $(x,y) \in \A \times \C$ such that their
patterns of zeroes are ``similar'', and progressively restricting this
set, we will finally ensure an isomorphism for every pair of random
sequences. For this, we now introduce the notion of a
\emph{skeleton}. The skeleton of a finite string is the string we
obtain by mapping any non-zero symbol in it to a special character,
say $\text{\textvisiblespace}$. Consequently, if the patterns of 0s in
two finite strings $x \in \Sigma_A^*$ and $y \in \Sigma_C^*$ are
identical, then their skeletons will be identical. In this subsection,
we prove an effective version of Keane and Smorodinsky's Skeleton
Lemma \cite{KeaneSmorodinsky79} (see also Chapter 6, Lemma 5.3 in
Petersen\cite{Petersen89}). What goes in the blank spaces is called a
filler.

The strategy that we will adopt in the isomorphism is to map sequences
$x \in \Sigma_A^\infty$ to sequences $y \in \Sigma_C^\infty$ with
identical skeletons. The first stage in the construction will be to
identify the set of potential pairs of infinite sequences with
identical skeletons. To this end, we now define the notion of a
skeleton of rank $r$, $r \in \N$, and show that Martin-L\"of random
sequences in any system have skeletons of all ranks. Owing to the fact
that we have only approximation of probabilities of mixing Markov
systems, we consider a different setting for skeletons and later,
their fillers, from the one considered in \cite{KeaneSmorodinsky79}
for Bernoulli process.


Assume that we have a sequence of positive integers $N_0 < N_1 <
\dots$. (This sequence will be fixed when we discuss the filler lemma,
where we establish that it can be computed layerwise.) For a skeleton
of rank $r$ centered at position $i$ in a sequence $x$, we look for
the shortest substring centered at $x[i]$ starting and ending with
$N_r$ (or more) consecutive $0$s. We replace all non-zero symbols with
blanks. We further replace the blocks of $0$s shorter than $m$ with
blanks.
\begin{definition}
Let $x \in A^\Z$. A \emph{skeleton $S_{x,r,i}$ of rank $r$ in $x =
  [.....x_{-2} x_{1} x_{0} x_{1} x_{2}.....]$} is defined as
follows. Starting from $x[i]$, pick the shortest string of the form
$0^{n_0} \text{\textvisiblespace}^{\ell_1}
0^{n_1}\ \dots\ \text{\textvisiblespace}^{\ell_k}0^{n_k}$ such that
the following hold.
\begin{itemize}
\item Each $\ell_i$ is at least 1, $(1 \le i \le k)$.
\item Each $n_i$ is at least $m$, $(1 \le i \le k)$.
\item $n_i < N_r$ for all $1 \le i \le k-1$. Further, both $n_0$ and
  $n_{m}$ are greater than or equal to $N_r$.
\end{itemize}
%% Then $S_{x,r,i}$ is the string $0^{n_0}
%% \text{\textvisiblespace}^{\ell_1}0^{n_1}
%% \text{\textvisiblespace}^{\ell_2}0^{n_2}
%% \dots
%% \text{\textvisiblespace}^{\ell_k}
%%   0^{n_k}$
\end{definition}
Note that blocks of zeroes of length less than $m$ are converted to
spaces. Thus, except for the extremities of the skeleton of rank $r$,
there is no contiguous block of $0$s longer than $N_r$. Also, it is
routine to see that a rank-$r$ skeleton can be uniquely decomposed
into skeletons of rank $r-1$ \cite{Petersen89}.


We now show that the skeleton of every Martin-L\"of random object in
has skeletons of every rank $r$ (with respect to any predetermined
sequence $N_1 < N_2 < \dots$ of numbers) while having sufficiently
many blanks in between. This is an effective version of the Skeleton
Lemma in \cite{KeaneSmorodinsky79}.

\begin{definition}
The \emph{length of the skeleton} $S_{x,r,i}$, denoted
$\ell(S_{x,r,i})$, is defined as follows.
$$\ell(S_{x,r,i}) = \left|\lbrace i \mid x_{i} \neq 0,\quad i \in
S_{x,r,i}\rbrace\right|$$
\end{definition}



%---------------------
% Skeleton Lemma v2
%---------------------
%% \begin{lemma}[Skeleton Lemma]
%% \label{lemma:skeleton}
%% Let $\{L_r\}_{r=0}^{\infty}$ be an increasing sequence of positive
%% integers. For every Martin-L\"of random $x$ there is a sequence $N_0 <
%% N_1 < \dots$ of positive integers computably enumerable with respect
%% to $x$ such that
%% \begin{itemize}
%% \item For every $r \in \N$, $S_{x,r,0}$ is delimited by a block of 0s
%%   of length at least $N_r$, and
%% \item For large enough ranks $r$, $S_{x,r,0}$ has at length at least 
%% $L_r$.
%% \end{itemize}
%% \end{lemma}


\begin{lemma}[Layerwise Skeleton Lemma]
\label{lemma:skeleton}
Let $\langle L_r \rangle_{r=1}^{\infty}$ be an increasing sequence of
positive integers. Then there is a layering $\langle K'_r
\rangle_{r=1}^\infty$ of $\A$ and an increasing sequence of positive
integers $\langle N_r \rangle_{r=0}^\infty$ uniformly computably
enumerable in $\langle K'_r \rangle_{r=1}^\infty$ such that for every
$r \in \N$ and every $x \in K'_r$, the following hold.
\begin{itemize}
\item There is a skeleton centered at $x[0]$ delimited by $N_r$ many
  zeroes.
\item The central skeleton centered at $x[0]$ and delimited by $N_r$
  many zeroes, has length at least $L_r$.
\end{itemize}
\end{lemma}

We prove the case when $m=1$. The general case is similar.
\begin{proof}
Define $K'_r = \{ x \in X \mid \ell(S_{x,r,0}) \ge L_r \}$. (Note that
in this step, we choose $N_1, \dots, N_r$ to determine the rank-$r$
skeleton.)Thus $K'_r$ contains all points $x$ such that their
``central skeleton'' of rank $r$ contains at least $L_r$ many spaces.

Consider
$$K' = \cup_{n=1}^{\infty} \cap_{r=n}^{\infty} K'_r,$$ the set of
points in $X$ such that for large enough ranks $r$, a skeleton of rank
$r$ contains at least $L_r$ many non-zero symbols. We form a layerwise
lower semicomputable function which attains infinity on each element
in $K'^c$.

Any $x$ in $K'^c$ has either of two properties -- first, $x$ does not
have any skeleton of rank $r$ (or above), and second, for every $n$,
there exists some rank $r \ge n$ such that $x$ has a central skeleton
having less than $L_r$ many spaces. We will form layerwise integrable
functions which will attain $\infty$ on $x$ in either of these cases.

{\bf Case I.} Suppose $x$ has no central skeleton of rank $r$ or
more. By the pigeonhole principle, there is some rank $r'<r$ such that
a rank $r'$ skeleton appears infinitely often in $x$. Suppose $r'$ is
the highest rank which appears infinitely often in any skeleton of
$x$, including non-central skeletons.

Let the left zero extremity (analogously, the right zero extremity) of
a string $w$ be the longest block of zeroes at the left end
(correspondingly the right end) of $w$. (These may, of course be
empty.) Let $ZE: \Sigma_A^* \to \{0\}^*$ be the function which returns
the shorter among the left zero extremity and right zero extremity.

Consider the following function defined on cylinders of $A^\Z$. The
function $f: A^* \to [0,\infty)$ is defined by
\begin{align*}
f(\lambda) &= 1\\
f(a_1\ w\ a_2) &= \begin{cases}
                 \frac{1}{(1-P_A(00\mid w))} f(w) &\text{ if } |ZE(w)|=N_{r'}
                 \text{ and } a_1a_2 \ne 00\\
                 0                       &\text{ if } |ZE(w)|=N_{r'} 
                 \text{ and }	  a_1a_2 = 00\\
                 f(w)                    &\text{ otherwise}
                 \end{cases}
\end{align*}

Define the function $S: A^\Z \to [0, \infty)$ by $S(x) = \sup_{n}
  f(x[-n \dots 0 \dots n])$. Since $P_A$ is computable, we can
  conclude that $S$ is layerwise lower semicomputable.

For infinitely many $n$, a skeleton of rank $r'$ will appear as the
extremities of $x[-n\dots 0 \dots n]$. Hence the subsequent bits on
the left and the right cannot both be 0. In this case, $f(x[-n-1\dots
  0 \dots n+1]) > f(x[-n \dots 0 \dots n])$. Thus, $S(x) = \infty$.

We observe that $\int f(\lambda) dP_A = 1$, viewing $f(\lambda)$ as a
constant function defined on every $x \in X$. Similarly, on any
cylinder $w$, if $w$ does not have extremities of the form $0^{N_r}$,
then $f(a_1 w a_2) = f(w)$, and we have
$$\sum_{a_1 a_2 \in \Sigma_A^2} f(a_1 w a_2) P_A(a_1a_2 \mid w) = f(w)
\sum_{a_1a_2 \in \Sigma_A^2} P_A(a_1a_2 \mid w),$$ which is $f(w)$. If
$w$ ends in extremities of the form $0^{N_r}$, then
$$\sum_{a_1 a_2 \in \Sigma^2\setminus \{00\}} f(a_1 w a_2) P_A(a_1 a_2
\mid w) = f(w) \frac{[1-P_A(00\mid w)]}{1-P_A(00\mid w)},$$ which is
$f(w)$ as well. So we have that
$$f(w) P_A(w) = \sum_{a_1a_2 \in \Sigma^2} f(a_1\ w\ a_2)
P_A(a_1\ w\ a_2).$$

Thus, we can see that
$$\int S(x) dP_A = \int \limsup_n f(x[-n \dots 0 \dots n]) dP_A
\le\sup_n \int f(x[-n \dots 0 \dots n]) dP_A= 1,$$ where the
inequality follows by Fatou's lemma.

{\bf Case II.} Now suppose that for every $n$, there is a central
skeleton in $x$ of rank $r \ge n$ such that $\ell(S_{x,r,0}) <
L_r$. This implies that within at most $L_r (N_r - 1)$ characters
around $x_0$, the block $0^{N_r}$ will occur in $x$. 

Consider the function $g_r: A^* \to [0,\infty)$ defined by
\begin{align*}
g^k_r(\lambda) &= \frac{1}{2^r L_r(N_r-1)}\\
g^k_r(a_1\ w\ a_2) &= \begin{cases}
  \frac{1}{P_A(00 \mid w)} g_r(w) 
  &\text{ if } k \le |w| < N_r \text{ and } a_1 a_2 =00\\ 
  0 &\text{ if } k \le |w| < N_r \text{ and} a_1 a_2 = 00\\
  f(w) &\text{otherwise.}
  \end{cases}
\end{align*}

As in case I, we can verify that for all cylinders $w$,
$$g^k_r(w)P_A(w) = \sum_{a_1a_2 \in \Sigma^2} g^k_r(a_1\ w\ a_2)
P_A(a_1\ w\ a_2).$$

Consider the function $g_r: A^* \to [0,\infty)$ defined by
$$g_r = \sum_{k=1}^{L_r(N_r-1)} g^k_r.$$

We know that if $x$ has a deficient rank $r$ at length $k$, then 
$$g_r(x) \ge \frac{1}{2^r} \frac{1}{L_r (N_r-1) P_A(0)^{N_r}} \ge 1$$
if we choose large $N_r$ in a suitable manner.

Finally, consider the aggregate function $S : A^\Z \to [0,\infty)$
  defined by $S= \sup_n \sum_{r=1}^{\infty} g_r$. Then, as in case I,
  we see that $S$ is layerwise lower semicomputable and
  integrable. Since by assumption $x$ has infinitely many $r$ for
  which $g_r$ attains at least $1$, we have that $S(x) = \infty$.
\end{proof}

We will now proceed to choose this sequence of $L_r$s that is assumed
in Lemma \ref{lemma:skeleton}.

%% TeX-Master=markov.tex
 

%%  LocalWords:  Smorodinsky's layerwise semicomputable ZE dP Fatou's


==> 5.filler_lemma.tex <==
\subsection{Effectively determining $L_r$ and Filler lemma}
In the last subsection, we assumed that we have a sequence $L_0 < L_1
< \dots$ of natural numbers. For every $i, r \in \N$ and $x \in \A
\cup \C$, a skeleton in $x$ of rank $r$ at position $i$ was the
shortest string centered at $x[i]$ and delimited by the earliest
appearance of $N_r$ many zeroes and at least $L_r$ many spaces. We now
see how we determine this sequence in a layerwise lower semicomputable
manner.

We define a sequence of $\langle L_r\rangle_{r=1}^\infty$ for the
lengths of the skeletons of rank $r$ inductively. We choose the
sequence $\langle N_i \rangle_{i=1}^{\infty}$ such that a skeleton of
rank $r$ has length at least $L_r$. We compute the lengths $L_r$
layerwise, in such a way that properties analogous to the asymptotic
equipartition property hold for the skeletons of rank $r$ for every
Martin-L\"of random sequence. This will allow us to construct a
provably isomorphic map between \A and \C.

Let $\eta_r=\min_{i\in\{A,C\}}\min_{\substack{a\in\Sigma_i,
    b\in\Sigma_i^m}} P_i(a \mid b,r)$. Similarly, let $\theta_r =
\max_{i\in\{A,C\}}\max_{\substack{a\in\Sigma_i, b\in\Sigma_i^m}} P_i(a
\mid b,r)$.  We want a strictly increasing sequence $\langle
L_r\rangle_{r=1}^\infty$ such that:\footnote{Note that here we deviate
  from the original construction. Without loss of generality, $\eta_r>0$
  -- since if a $m+1$ length sequence of alphabets has probability $0$,
  we can safely ignore those strings as we are required to succeed only
  in a measure 1 subset.}
$$\lim_{r\to\infty}
\frac{1}{\eta_r}2^{-L_r(\varepsilon_{r-1}-\varepsilon_r)}=0.$$ Note
that $L_r=3+r$ is such a sequence -- since $\frac{1}{\eta_r}\le
\frac{1}{\eta (1-\varepsilon_r)}$ where $\eta$ is minimum non-zero
conditional probability and
$\varepsilon_{r-1}-\varepsilon_r=\varepsilon_r$. In the following, we
assume $L_r=3+r$. We use this specific value in lemma
\ref{lem:filler-lem}
%% But we can still find such
%%$L_r$ because of the right quantifier alternation.
%Also we don't know $k_r$ and hence we can't compute $L_r$. But our
%construction of isomorphism works ( and gives same map ) for any
%$\{L'_r\}$ sequence which has property $2$ and majorizes
%$\{L_r\}$. So, we can dovetail over prefixes of candidate
%$\{L_r\}$-sequences while constructing the isomorphism between \A and
%\C.

Let $S$ be a skeleton of length $\ell$ and rank $r$. So, the filler
for $S$ in \A is $\Sigma_{A}^\ell$ and in \C is
$\Sigma_{C}^\ell$.\footnote{In contrast with
  \cite{KeaneSmorodinsky79}, we include 0s in our filler alphabets.}
For the moment let us only consider the system \A -- similar is done
for \C in order to construct the isomorphism.

Let $S$ be a skeleton of length $\ell$ and rank $r$. Let $\F(S)
\subseteq \Sigma_A^\ell$ denote the set of fillers for $S$ in \A.  Let
$Z_S$ denote the indices of $0$s in $S$ and let the blanks be in
positions $s_1,s_2,\dots s_\ell$. Note that $Z_S$ does not
contain indices of a $0$ block shorter than $m$.

Given a filler $F\in\F(S)$ and an index set $I \subseteq \{s_1, s_2,
\dots, s_\ell\}$ over the blank places of $S$, let $\langle I,F,S
\rangle$ denote the cylinder generated by setting $0$s from $S$ and
setting $i^{th}$ position for $i \in I$ with the corresponding
symbol in the filler $F$.

Now, for an $n \in \N,n\ge r$,\footnote{We define $J(F,n)$ only when 
$n\ge r$} we define an equivalence relation $\sim_n$ for
error bound $\varepsilon_n$ on $\F(S)$ and denote equivalence class of
$F$ by $\tilde{F}_n$. We decide a subset of places $J(F,n) \subseteq
\{s_1, s_2,\dots, s_\ell\}$ for each $F$ and declare $F\sim_n F'$ if
$J(F,n)=J(F',n)$ and $F$ agrees with $F'$ on $J(F,n)$.
%{\bf Changelog: $r$ to $n$ because $r$
%  is the rank of the skeleton. Please verify the following
%  description, with $r$ and $z$ replaced with $n$.}

For a fixed $n\ge r$ and $F$,
we define $J$ inductively on the rank of the skeleton. 
%% For convenience of notation, for any positive integer $m$, denote the
%% set $\{1, 2, \dots, m-1\}$ by $\llbracket m \rrbracket$.

For a skeleton $S$ of rank 1 and length $\ell$, we proceed as
follows. Pick the largest positive integer $k$, $k \le \ell$ such that 
$$P_A(\ \langle\{s_1,s_2,\dots,s_k\},F,S\rangle,\ n\ )\ \ \ge\ \ \frac{3}{2\eta_1} 
2^{-(\ell+|Z_S|)(H-\epsilon_1)}.$$ Then, let $J(F,n) = Z_S \cup \{s_1,
s_2, \dots, s_k\}$.

Now, for a rank $r\ge 2$ skeleton $S$ and $F\in\F(S)$, we do the
following: Let us assume that $S=S_1\times S_2\times \dots \times S_t$
is the skeleton decomposition of $S$ where each $S_i$ is of rank
$r-1$. Also let $F_1,F_2,\dots,F_t$ are the corresponding fillers
which coincides with $F$. We assume that we have determined $J(F_i, n\log 3t)$
inductively for each $F_i$.
%It is possible to do this, since we have an upper bound of $n(\log 3t)^r$
%precision to do the entire computation. 

Let $J_0(F,n)=\cup_{i=1}^t J(F_i, n\log 3t)$.\footnote{The purpose of $n\log 3t$
will be clear in lemma \ref{lem:prod-of-society}}
%(here we abuse the notation: $J(S_i, n\log 3t)$ refers to corresponding
%places in $S$, rather than those in $S_i$).
These are the positions in $S$ which have already been determined in the
previous rank.

Also, let $\{s_1,\dots s_\ell\}\setminus J_0(F,n) =\{t_1\dots t_u\}$, where
$t_1<\dots <t_u$. These are the positions in the skeleton $S$ which
have not been fixed by any rank $r-1$ subskeletons. Then, we set
$J(F,n)=Z_S\cup J_0(F,n)\cup\{t_1,\dots,t_k\}$, where $k \le u$ is the
largest positive integer such that
$$P_A(\ \langle\{t_1,\dots t_{k-1}\}\cup J_0(F,n), F,S \rangle, n\ )\ \ \ge\\
\ \frac{(1+\varepsilon_r)}{\eta_r}2^{-(\ell+|Z_S|)(H_{}-\varepsilon_r)}.$$
Note that we allow $J(F,n)$ to be $Z_S\cup \{s_1,s_2,\dots,s_l\}$ and 
$\eta_r/(1+\varepsilon_r)$ is a pessimistic approximation of true minimum
conditional probability of an alphabet.

Let $x=0^{l_1}x_10^{\ell_2}x_20^{\ell_3}\dots 0^{\ell_{t}}
x_{t}0^{\ell_{t+1}}$ be a string where $\ell_i>m$ for all $1\le i\le
t+1$.  Let
$$P'_A(x,n)=\frac{\prod_{i=1}^t
    P_A(0^{\ell_{i}}x_i0^{\ell_{i+1}},n\log 3t)}{\prod_{i=2}^t
    P_A(0^{\ell_i})}.$$
By the Markov property, we have that
$$
P_A(x) = P_A\left(0^{\ell_1} x_1 0^{\ell_2}\right) \prod_{i=2}^{t}
P\left(x_i 0^{\ell_{i+1}} \mid 0^{\ell_1} x_1 \dots
0^{\ell_i}\right) = P_A\left(0^{\ell_1} x_1 0^{\ell_2}\right)
\prod_{i=2}^{t} P\left(x_i 0^{\ell_{i+1}} \mid 0^{\ell_i}\right).
$$
Hence,
\begin{equation}
\label{eqn:probmult}
  \left|P_A(x)-P'_A(x,n)\right|\le \varepsilon_n P'_A(x,n).
\end{equation}

So, $P'_A(x,n)$ can be used in place of $P_A(x,n)$ but for the fact we
cannot compute $P_A(0^{\ell_i})$ exactly. But we use the essentially
multiplicative nature of $P'_A$  and that it approximates $P_A()$ 
in the proof of lemma \ref{lem:prod-of-society}.  The approximation
is as follows: $|P_A(x,n)-P'_A(x,n)| \le 2\varepsilon_r P_A(x,n)$.

Also, we note that for a given $F\in\F(S)$ and an integer $n$,
$J(F,n)\subseteq J(F,n+1)$. In other words, if we decrease the error
bound in estimation of probability the equivalence relation can only
get finer.

Similar relations holds for \C.

%\{Comment: $P_i ( a \mid b, r')$ changed.\}

Note that $\theta_r$ and $\eta_r$ is bounded from below and above with
respect to $r$ for a mixing Markov process. Then we have the following
bounds.
\begin{lemma}[Filler Lemma]
  \label{lem:filler-lem}
  There is a layering $\langle K''_p\rangle_{p=1}^\infty$ such that or
  every $n$, there is a large enough $r$ such that for every skeleton
  $S$ of rank $r$ and length $\ell$ corresponding to $x\in K''_r$, we
  have:
  \begin{enumerate}
    \item For all $F\in\F(S)$, $P_A\left(\tilde{F}_r,n\right)\ge
      (1-\varepsilon_n)2^{-L(H-\varepsilon_r)}$
    \item For all $F\in\F(S)$ except maybe on a set of measure
      $\varepsilon_n$:
      \begin{enumerate}
      \item
        $P_A(\tilde{F}_r,n) <
        \frac{1+\varepsilon_n}{(1-\varepsilon_r)^2}\frac{1}{\eta_r}
        2^{-L(H_{}-\varepsilon_r)}$
	\item $\frac{1}{L}|J(F,r)| > 1-\frac{3}{|\log_2
          \theta_r|}\varepsilon_r$
      \end{enumerate}
  \end{enumerate}
   where $L=\ell+|Z_S|$.
\end{lemma}
\begin{proof}
%   Let $p'$ denote an integer such that $\varepsilon_{p}\le 2H\varepsilon_{p'}$.
  From the effective Shannon-McMillan-Breiman theorem, we know that
  there is a layering $\langle K''_p\rangle_{p=1}^\infty$ such that for
  all $p$ there is a $k_p$ so that for all $k\ge k_p$,
  $\Sigma_{A}^k=K''_p\cup (K''_p)^c$, with the following properties:
\begin{itemize}
  \item $P_A(K''_p)\ge 1-\varepsilon_{p}$
  \item For each $x\in K''_p$ we have 
$$\frac{1+\varepsilon_p}{\eta_p}2^{-k(H_{}+\varepsilon_{p})}< P_A(x,p)<
    \frac{1-\varepsilon_p}{\eta_p}2^{-k(H_{}-\varepsilon_{p})}.$$
\end{itemize}
Now given an $n$, let $r\ge n+1$ be such that $L_r\ge k_n$.  Such an
$r$ exists, since $\{L_r\}$ is an increasing sequence.
\begin{enumerate}
\item Let $J(F,r)=Z_S\cup J_0(F)\cup\{t_1,t_2\dots t_w\}$. Then 
  \begin{eqnarray*}
  P_A(\tilde{F}_r,n) & \ge & (1-\varepsilon_n)P_A(\langle
  J_0(F)\cup\{t_1,t_2\dots t_w\},F,S\rangle)\\ & \ge &
  \frac{1-\varepsilon_n}{1+\varepsilon_r}P_A(\langle
  J_0(F)\cup\{t_1,\dots,t_{w}\},F,S\rangle,r) \\ & \ge &
  \frac{1-\varepsilon_n}{1+\varepsilon_r}P_A(\langle
  J_0(F)\cup\{t_1,\dots, t_{w-1}\},F,S\rangle,r) \times
  P_A(F[t_w]|\langle
  J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,r)\\ & \ge &
  \frac{1-\varepsilon_n}{1+\varepsilon_r}\frac{1+\varepsilon_r}{\eta_r}2^{-L(H_{}-\varepsilon_{r})}
  \times P_A(F[t_w]|\langle
  J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,r)\\ & \ge &
  (1-\varepsilon_n)2^{-L(H_{}-\varepsilon_{r})}.
  \end{eqnarray*}
  where the inequality before the last follows from the definition of
  $J(F,r)$.
%   \begin{eqnarray*}
%   P_A(\tilde{F}_n,n) & \ge & (1-2\varepsilon_n)P'_A(\langle
%   J_0(F)\cup\{t_1,t_2\dots t_w\},F,S\rangle,n)\\ & \ge &
%   (1-\varepsilon_n)P'_A(\langle
%   J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,n) \times
%   P'_A(F_{t_w}|\langle
%   J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,n)\\ & \ge &
%   (1-\varepsilon_n)\frac{1}{\eta_r}2^{-L(H_{}-\varepsilon_{r})}
%   \times P'_A(F_{t_w}|\langle
%   J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,n)\\ & \ge &
%   (1-\varepsilon_n)2^{-L(H_{}-\varepsilon_{r})}.
%   \end{eqnarray*}

\item
  \begin{enumerate}
  \item If $|J(F,r)|<L$, then by the definition of $J(F,r)$, we
    have $$P_A(\tilde{F}_r,n)\le (1+\varepsilon_n)P_A( \tilde{F}_r)
    \le\frac{1+\varepsilon_n}{1-\varepsilon_r}
    P_A(\tilde{F}_r,r)<\frac{1+\varepsilon_n}{1-\varepsilon_r}\frac{1+\varepsilon_r}{\eta_r}
    2^{-L(H_{}-\varepsilon_r)}<\frac{1+\varepsilon_n}{(1-\varepsilon_r)^2}\frac{1}{\eta_r}
    2^{-L(H_{}-\varepsilon_r)}$$ If $|J(F,r)|=L$, then
    $\tilde{F}_r=F$. But $|F|=L\ge L_n\ge k_n$ and hence $$P_A(F,n)\le
    (1+\varepsilon_n)P_A(F) \le
    \frac{1+\varepsilon_n}{1-\varepsilon_r}P_A(F,r)
    <\frac{1+\varepsilon_n}{\eta_r} 2^{-L(H_{}-\varepsilon_r)}$$
    unless $F\in (K''_r)^c$ and
    $P_A((K''_r)^c)<\varepsilon_r<\varepsilon_n$.
  \item Without loss of generality, assume that (a) holds.  (Otherwise
    we already have that such $F$ has to be in $\varepsilon_r$ measure
    set.) Let $L-|J(F,r)|\ge 3L\varepsilon_r/|\log_2 \theta_r|$. Then,
    \begin{eqnarray*}
      P_A(F,n)&\le& \frac{1+\varepsilon_n}{1-\varepsilon_r}P_A(F,r)
      \\ 
      &\le& \frac{1+\varepsilon_n}{1-\varepsilon_r} P_A(\tilde{F}_r,r) \times
      \prod_{i\not\in J(F,r)} P_A(F[i]|\langle 
      J_0(F)\cup\{t_1,\dots,t_{w-1}\},F,S\rangle,r)\\  
      &\le& \frac{1+\varepsilon_r}{1-\varepsilon_n} P_A(\tilde{F}_r,r) \cdot
      \theta_r^{3L\varepsilon_n/|\log_2 \theta_r|} \le 
      \frac{1}{(1-\varepsilon_n)^2(1-\varepsilon_r)^2}
      \frac{1+\varepsilon_r}{\eta_r}2^{-L(H_{}-\varepsilon_r)}2^{-3L\varepsilon_r}\\  
      &\le&\frac{2^{-L\varepsilon_r}}{(1-\varepsilon_n)^2(1-\varepsilon_r)^2}
      \frac{1+\varepsilon_r}{\eta_r}2^{-L(H_{}+\varepsilon_r)}
      \le\frac{1+\varepsilon_r}{\eta_r}2^{-L(H_{}+\varepsilon_r)} .
    \end{eqnarray*}
    Here the last inequality follows from $L_r=3+r$. We also use the
    inequalities $\frac{1+\varepsilon_n}{1-\varepsilon_r} 
    < \frac{1+\varepsilon_r}{1-\varepsilon_n}$ and $\theta^{1/|\log_2
      \theta|}\le 2^{-1}$. 
    In this case $F$ must belong to the set $(K'_r)^c$ 
    of measure less than $\varepsilon_r$.  Hence the set on which $L$
    can violate the bound has measure 
    $<2\varepsilon_r\le \varepsilon_n$.
  \end{enumerate}
\end{enumerate}
\end{proof}

%% TeX-Master=markov.tex
 

%%  LocalWords:  layerwise semicomputable indices subskeletons
%%  LocalWords:  Breiman

